GCS: Graph-based Coordination Strategy for Multi-Agent Reinforcement Learning

Many real-world scenarios involve a team of agents that have to coordinate their policies to achieve a shared goal. Previous studies mainly focus on decentralized control to maximize a common reward and barely consider the coordination among control policies, which is critical in dynamic and complicated environments. In this work, we propose factorizing the joint team policy into a graph generator and graph-based coordinated policy to enable coordinated behaviours among agents. The graph generator adopts an encoder-decoder framework that outputs directed acyclic graphs (DAGs) to capture the underlying dynamic decision structure. We also apply the DAGness-constrained and DAG depth-constrained optimization in the graph generator to balance efficiency and performance. The graph-based coordinated policy exploits the generated decision structure. The graph generator and coordinated policy are trained simultaneously to maximize the discounted return. Empirical evaluations on Collaborative Gaussian Squeeze, Cooperative Navigation, and Google Research Football demonstrate the superiority of the proposed method.

==> 2-preliminary.tex <==
% \section{Preliminary}
\section{Problem Setup}
% a convenient mathematical model to solve sequential decision-making problems under imperfect observations.
% \subsection{Decentralized Partially Observable Markov Decision Processes}

\paragraph{\textbf{Dec-POMDPs.} }
\added{We consider a cooperative multi-agent system ***}
The Decentralized Partially Observable Markov Decision Processes (Dec-POMDPs)~\cite{oliehoek2016POMDPs}
% ~\citep{hu1998multiagent,littman1994markov}
\deleted{is the generalization of POMDP for dealing with sequential decision-making problems of $N$ agents}
% \replaced{They}{Dec-POMDPs} 
, which can be expressed as a tuple 
$<\{\mathcal{I}\}, \mathcal{S}, \{\mathcal{O}^i\}_{i=1}^N, $ \\ $\{\mathcal{U}^i\}_{i=1}^N, \mathbb{P},r>$.
$i \in \mathcal{I}$ is the $i^{th}$ player, 
$\mathcal{S}$ is the global state space, 
$\mathcal{O}^i$ and $\mathcal{U}^i$ denote the observation space and the action space for the $i^{th}$ player,  respectively. 
We label 
% We \replaced{label}{let}
$\bm{u}:=(u^1,...,u^N)$
% \replaced{}{denote} 
the joint actions for all players. 
$\mathbb{P}$ is the transition dynamics, and $\mathbb{P}(\cdot |s,\bm{u})$ gives the distribution of the next state at state $s$ taking action $\bm{u}$. 
All agents share the same reward function $r(s,\bm{u}):s \times \bm{u} \to R$. 
% $r^i$ is the reward function for the $i^{th}$ player after taking the joint action $\bm{u}$.
% \replaced{Label}{Let}
$\gamma \in (0,1)$
% \replaced{}{denote} 
denote a discount factor and $\tau  = ({s_0},{\bm{u}_0},{s_1},...)$ 
% \replaced{}{denote} 
denote the trajectory induced by the policy $\pi=\{\pi^i\}_{i=1}^N$. All the agents coordinate
together to maximize 
% \replaced{maximize}{maximizes} 
the cumulative discounted return ${\mathbb{E}_{\bm{\tau}  \sim \pi }}\left[ {\sum\nolimits_{t = 0}^\infty  {{\gamma ^t}r({{s}_t},{\bm{u}_t})} } \right]$.

\paragraph{\textbf{Dec-POMDPs with action coordination graph.}} 
We formalize our problem under Dec-POMDPs
and optimize an action coordination graph to represent
% \replaced{and optimize an}{to find the optimal} 
% action coordination graph to represent}{representing} 
the hierarchical action dependency structure {for better coordination} among all agents.
Different from Dec-POMDPs, where all actions are taken simultaneously and do not depend on each other, we endow the hierarchy order to the joint action based on the learned DAG structure $\mathcal{G}$, called ACG.
The adjacency matrix $A$ representing the ACG  denotes the hierarchical action dependency from the graph generation policy $\rho$.
% $\mathcal{G}$ from the graph generation policy $\rho$ denotes the hierarchical action dependency at time $t$.
Therefore, we can define ${\pi _{{\theta ^i}}}({u^i}|{o^i},{u^{pa(i)}})$ as the hierarchical decision policy for the $i^{th}$ player, where $pa(i)$ is the parents of agent $i$ and ${u^{pa(i)}}$ is the actions taken from the parents, whose order is generated from $A$. 
% whose order is generated from the directed acyclic graph. 
Note that fully decentralized policy is a special case of our hierarchical decision policy where all the agents have no parents. Correspondingly, the graph $\mathcal{G}$ is a scatterplot, and the adjacency matrix $A$ is a zero matrix.
Moreover, in our setting, the state-action value function is denoted as
% \begin{equation}
$$
{Q^\pi }(s,{\bm{u}^{A \sim \rho }}) = {\mathbb{E}_{\pi ,\rho }}\left[ {\sum\limits_{k = 0}^\infty  {{\gamma ^k}r({s_{t + k}},{u_{t + k}})|{S_t} = s,{A_t} = {\bm{u}^{A \sim \rho }}} } \right].
$$

% \yali{$A$ or $\mathcal{G}$? consistency}
We propose that the DAG $\mathcal{G}$ can be regarded as the underlying decision structure of MAS due to its natural properties\footnote{Since the hierarchical action dependency among agents is orderly(directed) and the execution of action is one-time (acyclic) at each timestep $t$, DAG is a natural and excellent structure to represent the underlying structure of the hierarchical action dependency among agents.}.
% Note that 
As shown in Figure~\ref{fig:demo-topo}, we give an illustrative description of the DAG and the relationship between nodes. 
% It shows the hierarchical dependency clearly.
% We regard the graph $\mathcal{G}$ as the underlying decision structure of MAS. 
The nodes in $\mathcal{G}$ correspond to the agents in MAS, and the parent-child relationship represents the hierarchical action dependency among agents.
% \replaced{represents}{in $\mathcal{G}$ is used to represent} the hierarchical action dependency among agents\replaced{}{ in MAS}.
% For example, the case that node $A$ in the graph has no parents represents agent $A$ take action independently.
For example, the case that the node $D$ in the graph has two parents $\{B,C\}$ illustrates the action taken by the agent $D$ constrained by $B$ and $C$.



% and node $D$ is the parent of vertexes $B$ and $C$. Therefore, traversing the topological order $\{A,B,C,D,E\}$ of $\mathcal{G}$, we can get the dependency relationship for each vertex.
% and the parent-child relationship among agents.
% \yali{)$pa(i)$ is not defined. ii) $\mathcal{G}$ is not clear too.
% iii) adding an illustrative graph will be helpful.}
% \end{equation}



% \yali{First, we need to introduce POMG. Second, I would suggest using POMDP instead of POMG, because in our setting all agents are collaborating and share rewards. Markov game is usually for individual reward setting. }
% \jqruan{to yali: Already corrected it.}

% \subsection{Directed Acyclic Graphs}
% A graph is a series of vertexes connected by edges in graph theory. The Directed Acyclic Graphs (DAGs)~\citep{thulasiraman19925, bang2008digraphs} with $N$ vertices can be described as a graph that the edges are directed going from one node to another, and no cycles are connecting the other edges. A key property of DAGs is topological ordering, which means we can use a linear ordering to represent the relationship of the nodes in DAGs. That is, topological ordering is to arrange all vertices in DAGs into a linear sequence, so that any pair of vertices $u$ and $v$ in the graph, if the edge $(u, v) \in Edges(G)$, then $u$ appears before $v$ in the linear sequence.
% For example, a topological ordering of the DAGs is shown in Fig.\ref{fig:demo-topo}.

\begin{figure}[ht!]
    \centering
      \includegraphics[width=0.9\linewidth]{fig/topological.pdf}
% 	  \caption{The schematic diagram of converting a directed acyclic graph $\mathcal{G}$ with vertices $|\mathcal{V}|=5$ and edges $|\mathcal{E}|=7$ into a topological sorted graph $\mathcal{G}_t$. One of the topological ordering for $\mathcal{G}$ is $\{A,B,C,D,E\}$}
\caption{The left is the schematic diagram of a directed acyclic graph $\mathcal{G}$ with vertices $|\mathcal{V}|=5$ and edges $|\mathcal{E}|=7$. The right is the parent-child relationship about $\mathcal{G}$.}
	  \label{fig:demo-topo}
\end{figure}

% demo-topological



==> legacy.tex <==


\section{Related Work}
% rl -> marl
\added{Deep reinforcement learning has demonstrated its success in addressing complex decision problems \citep{silver2017alphagozero,schrittwieser2020muzero}.
}
\deleted{Recently, advances~\cite{silver2017alphagozero,schrittwieser2020muzero,chen2020conditional} in deep reinforcement learning have demonstrated its potential to address complex decision problems, and consequently, the 
widespread existence of multi-agent systems (MAS) in the real world has further catalyzed the emergence of multi-agent reinforcement learning (MARL)~\cite{du2021survey,yang2020overview}. }
\added{Due to the wide existence of multi-agent tasks, MARL has attracted wide attention.}
\added{Based on information structures, we classify the existing approach into three categories.}

% 2nd CTDE
\replaced{centralized training with decentralized execution considers ***}{
Solutions to effectively tackle multi-agent problems in MAS use \textit{centralized training with decentralized execution} (CTDE)~\cite{lowe2017maddpg} paradigm, which alleviates the non-stationarity from the decentralized approaches~\cite{tan1993iql} and the poor scalability from brought by the centralized methods.}
{Representative algorithms include \cite{lowe2017maddpg,foerster2018COMA,iqbal2019maac}.}
Some approaches~\cite{lowe2017maddpg,foerster2018COMA,iqbal2019maac} extend the actor-critic algorithm~\cite{degris2012actorcritic}, which embraces CTDE to train the actor to generate policies 
% \replaced{policies}{the policy} 
for each agent and use the centralized critic to evaluate them.
Moreover, a series of popularized value-based methods~\cite{sunehag2018vdn,rashid2018qmix,RashidFPW2020wqmix,son2019qtran,yang2020Qatten}
% \replaced{}{popularized recently} 
combined with the CTDE recently show great overwhelming superiority in MARL. 
% \replaced{We}{In our work, we} 
We develop an algorithm with value-based solutions under the CTDE regime due to its powerful capabilities.

% coordination
In MAS, the most fundamental problem is multi-agent coordination~\cite{busoniu2008comprehensive_survey}, and there is a rich literature of methods proposed to promote coordination. 
Here, we category these methods into two main parts. (a). \textbf{Communication-based methods}. Communication is the basis for efficiency and success in human society, and this fact 
% \replaced{and this fact}{which} 
is also applicable to the MAS. Some methods~\cite{foerster2016RIALDIAL,sukhbaatar2016CommNet,zhang2013coordinating,peng2017bicnet,jiang2018atoc,du2021flowcomm} 
% \replaced{}{are proposed to} 
autonomously learn communication protocols that are required in generating informative messages for coordination among agents.
(b). \textbf{ Non-communicative methods}. A large body of works {explores} how to infer actions of other agents for better coordination. 
% \jqruan{the following works are not suitable. find behavior reasoning}
Representative works include PR2~\cite{wen2019pr2}, GR2~\cite{wen2020gr2} and other-play~\cite{hu2020otherplay}, which aggregate information about other agents' decision patterns to promote the current policy. 
In addition, some works are devoted to tackling the credit assignment for overall coordination. For example, implicit methods include 
modeling the counterfactual policy gradient~\cite{foerster2018COMA}, learning intrinsic reward~\cite{du2019liir}, and explicit methods include value function decomposition~\cite{sunehag2018vdn,rashid2018qmix,son2019qtran}. Another line to promote coordination that is closely related to our approach is
to build a 
% \replaced{to build a}{the} 
coordination graph~\cite{guestrin2001cg,bohmer2020dcg,li2021dicg}, which aims to improve the value function estimates but
% \replaced{allows}{allow} 
allows explicit modeling of the locality of interactions. 
Similar but essentially distinct, we introduce a mechanism to learn the optimal DAG structure to model the dependencies among actions explicitly.
% \replaced{}{ using graph structures}. 
% \replaced{We introduce a similar but essentially distinct mechanism, which learns the optimal DAG structure to model the dependencies among actions in an explicit manner}{Similar but essentially distinct, we introduce a mechanism to learn the optimal DAG structure to model the dependencies among actions explicitly}. 
% \replaced{DAG}{directed acyclic graph (DAG)}


The generation of the DAGs is an essential part of our work. 
Recently, some continuous optimization approaches~\cite{zheng2018dagsnotears,yu2019daggnn,yu2020dagsnocurl,lachapelle2020gradientdag} have been proposed to recover the DAGs through structure learning. The method~\cite{zhu2019dagRL}, closely related to our work, uses reinforcement learning as its search strategy to maximize the predefined score function. Our work improves the DAG generation method~\cite{zhu2019dagRL} due to its natural advantage of perfectly fitting downstream reinforcement learning tasks.
\yali{what is the connection to our methods?}
% dag generation techniques
% The generation of the DAGs is an \replaced{essential}{important} part of our work. 
% Recently, some continuous optimization approaches~\cite{zheng2018dagsnotears,yu2019daggnn,yu2020dagsnocurl,lachapelle2020gradientdag} \replaced{have been}{are} proposed to recover the DAGs through structure learning. The method~\cite{zhu2019dagRL}\replaced{, closely related to our work,}{ is the most closely to our work, which} 
% uses reinforcement learning as \replaced{its}{the} search strategy to \replaced{maximize the}{obtain the largest} predefined score function. \replaced{Our work improves the DAG generation}{In our work, we improve the DAG generation method}~\cite{zhu2019dagRL} due to its natural advantage \replaced{of perfectly fitting}{that can perfectly fit our} downstream reinforcement learning tasks.

% most closely to our work is   
% Transforming the combinatorial optimization problem into a continuous equality constraint applied to linear structural equation model(SEM)~\cite{zheng2018dagsnotears} is the first step. DAG-GNN~\cite{yu2019daggnn} use the variational autoencoder as a deep generative model to to learn the DAG. 
% there is a large body of work on the scalability of
% There is a rich literature of algorithms proposed to tackle multi-agent problems~\cite{tan1993iql,sunehag2018vdn,rashid2018qmix,foerster2018COMA,iqbal2019maac}, which shows that the use of \textit{centralized training with decentralized execution}(CTDE)~\cite{lowe2017maddpg} paradigm 
% various methods are proposed to  
% the key development 
%  have recorded sublime success in various fields.
% gains rapid traction, and the latest accomplishments address problems with real-world complexity.
% In our work, we introduce a mechanism to generate explicit messages capturing relevant aspects of the world, which the agents are able to collectively learn using their observations and interactions.


% \replaced{}
\section{Methodology}

% \replaced{}{}
\deleted{
In this section, we give a novel problem formulation based on the MG framework and introduce the proposed framework that aims to learn an action coordination graph for policy training to implicitly promote coordination among agents. Then we further elaborate on the Decision Coordinator for graph generation and Policy Solver for policy training respectively.}
\yali{The message is not clear. It does no harm to delete it. }
% say, First, we give ***. Then, we introduce ***. }


% \subsection{Problem formulation}

\yali{hierarchical POMG should be explained earlier in Sec 3.}

We formalize our problem under the partially observable Markov Game (POMG) to find the optimal decision dependency structure among all agents for better coordination.
Different from POMG, where all actions are taken simultaneously and do not depend on each other, we endow the hierarchy order to the joint action based on the learned directed acyclic graph structure $\mathcal{G}_t$. 
The graph structure $\mathcal{G}_t$ denotes the optimal decision dependency at time $t$ and the policy ${\pi _{{\theta ^i}}}({u^i}|{o^i},{u^{pa(i)}})$ denote the decision policy for the $i^{th}$ player, where ${u^{pa(i)}}$ is the parents of $u^i$ generated by the directed acyclic graph. 
That is, we want to solve the following problem:
% \mathcal{G}
\begin{equation}
{\pi ^*},{\rho^*} = \mathop {\arg \max }\limits_{\pi ,\rho} {Q^\pi }(s,{\bm{u}^{\mathcal{G}\sim \rho}}){\ \ }s.t.{\ }\mathcal{G} \in DAGs{\rm{   }}.
\end{equation}
where ${Q^\pi }(s,{\bm{u}^{\mathcal{G}\sim \rho}}) = E\left[ {R_t^i|{s_t} = s,{u_t} = {\bm{u}^{\mathcal{G}\sim \rho}}} \right]$ is the state-action \replaced{value}{Q-function} and $\bm{u}^{\mathcal{G}\sim \rho}$ is the joint action whose decision dependency sequence is generated by $\mathcal{G}$. 



\subsection{\replaced{Multi-agent actor-critic}{Approach Overview} (better to use content words )}
Our goal is to learn an action coordination graph for generating the decision dependency sequence to promote policy training.  We can formulate the policy solving process as:
\begin{equation}
    \hat \pi (\bm{u},\hat A|s) = \prod\limits_{i = 1}^n {{\pi ^i}({u^i}|{o^i},{u^{pa(i) \sim \hat A}})\rho (\hat A|s)} 
\end{equation}
At the first step, we aim to find the optimal graph generation policy $\rho^*$ to obtain the DAG $\mathcal{G}$ that assigns agents a decision order $\hat A$. 
At the second step, we explore the the optimal action policy $\pi^*$ that obtains the final joint action sequence under the decision order $\hat A$ at every timestep $t$.
Then we optimize the two parts by maxmizing the cumulative return simultaneously.
% and the optimal action policy $\pi^*$ that obtains the final joint action sequence to optimize the cumulative return under the decision order $\hat A$ at every timestep $t$.
Fig.\ref{fig:overview} is the schematics of our solving framework. 
The decision coordinator, which is used to generate the action coordination graph, obtains the optimal graph policy to promote cooperation. The policy solver obtains the optimal decision policy based on the generated action coordination graph. Then we further elaborate on the decision coordinator and policy solver respectively.

\begin{figure}[th!]
\begin{center}
\includegraphics[width=0.8\linewidth]{fig/0-overall.png}
\end{center}
\caption{Overview of our framework.}
\label{fig:overview}
\end{figure}

\subsection{Decision Coordinator}

As shown in Fig.\ref{fig:graphgenerator}, the decision coordinator takes the local observations of the agents as input and outputs the Coordinator(Coord. for short) factor $\mathcal{G}$ for the decision-making process of the policy solver. 
Since the decision dependency among agents is orderly(directed) and the execution of action one-time (acyclic) at each timestep, DAG is a natural excellent structure to represent the underlying structure of decision-making process among agents.
Unlike the existing DAG generation methods~\cite{zheng2018dagsnotears,yu2020dagsnocurl,lachapelle2020gradientdag,yu2019daggnn} whose goal is to find the best DAG, we focus on exploring the optimal DAG generation policy. 
Inspired by the~\cite{zhu2019dagRL}, a DAG generation method using reinforcement learning, we adopt the actor-critic architecture as the decision coordinator to generate and evaluate the action coordination graph $\mathcal{G}$ through jointly training with the downstream tasks. 
We will elaborate on this module in the following.
% we improve it as the decision coordinator to generate the Coord. factor $\mathcal{G}$.
% Inspired by the~\cite{zhu2019dagRL}, a DAG generation method using reinforcement learning, we improve it as the decision coordinator to generate the Coord. factor $\mathcal{G}$ which is a directed acyclic graph. 
% The decision coordinator is a hot-swappable module, and you can use any DAG generation method to replace it. 
% But unlike the existing DAG generation methods~\cite{zheng2018dagsnotears,yu2020dagsnocurl,lachapelle2020gradientdag,yu2019daggnn} whose goal is to find the best DAG, we focus on exploring the optimal DAG generation policy.
% Motivated by recent advances in neural optimization~\cite{zhu2019dagRL}, we adopt the actor-critic architecture to generate and evaluate the action coordination graph through training with the downstream tasks jointly. 
% Different from~\cite{zhu2019dagRL} which aims to find the best DAG, we focus on exploring the optimal graph generation policy. 
% We use the external reward from the environment to evaluate the effectiveness of the graph structure under the exploitation and exploration scheme.
% the exploitation and exploration scheme in the RL paradigm provides an appropriate
% way to guide the search
% We use the external reward from the environment
% we attempt to use the external reward from the environment as a judgment of whether the graph structure promotes coordination among the agents. 

\begin{figure}[th!]
\begin{center}
\includegraphics[width=0.8\linewidth]{fig/0-Coord.png}
\end{center}
\caption{Schematics of the decision coordinator. The Coord. Actor including an encoder-decoder neural network model is used to generate the DAG from the observed data. 
% with some penalty terms to enforce acyclicity and maxmium depth, 
% which is then used to generate the topological order of the action sequence for interacting with the environments and obtain the optimal policy. 
The Coord. Critic is used to evaluate for useful and distinguishable graph structure by using the feedbacks from the downstream tasks.}
\label{fig:graphgenerator}
\end{figure}


\yali{suggest removing all abbreviations for ``Coord.". It is neither necessary nor clear.}
\textbf{\replaced{Coordination}{Coord.} Actor}.  The Actor contains two sub-modules. Firstly, we use the graph attention network (GAT)~\cite{velivckovic2018gat} as the attention-based encoder to extract the latent information for the graph structure generation. The simple feature is extracted by the multi-layer perceptron (MLP) as an initial step:
\begin{equation}
    {\{h_t^i\}}_{i=1}^N = f_{MLP}({\{o_t^i\}}_{i=1}^N, {\{u_{t-1}^i\}}_{i=1}^N).
\end{equation}

Due to the sufficiently expressive power, we further extract the latent information of the simple feature using GAT.
% To adequately extend the expressive power representing the latent information of the simple feature from MLP,
% find sufficiently expressive power representing the latent information of the raw observations, 
We compute the importance coefficients through the attention mechanism used in GAT:
\begin{equation}
    a_t^{ij} = \frac{{\exp (h_t^i\bm{W}{{(h_t^j\bm{W})}^T}/\sqrt {{d}} ))}}{{\sum\nolimits_{k \in {{\{ I\} }^{ - i}}} {\exp (h_t^i\bm{W}{{(h_t^k\bm{W})}^T}/\sqrt {{d}} )} }},\sum\nolimits_{j \in {{\{ I\} }^{ - i}}} {a_t^{ij}}  = 1,
    %  \vspace{1ex} 
\end{equation}
where $\bm{W} \in R^{d{'} \times d}$ is a learnable weight matrix, $d{'}$ and $d$ denote the dimension of the input vector and the latent vector respectively. $k \in {{\{ I\} }^{-i}}$ indexes other agents except the agent $i$.
Then multi-head attention is used to stabilize the learning process of self-attention and the final latent feature is as follows:
\begin{equation}
    h_t^{i'} = \sigma \left( {\frac{1}{K}\sum\limits_{i = 1}^K {\sum\limits_{j \in {{\{ I\} }^{ - i}}} {a_t^{ij}{\bm{W}^k}h_t^j} } } \right).
\end{equation}

Another sub-module in the Coord. Actor is the decoder that represents the process of generating a graph structure.
Since the GAT-based encoder has already provided sufficiently expressive features among the agents, the single-layer decoder is enough to easily construct the pairwise relationship between the encoder output and find a better structure of DAG for the optimal policy. 
\begin{equation}
    f_t^{ij}(\bm{h}_t^{l}, \bm{h}_t^{r}, u) = \sigma(u^Ttanh(\bm{W_l}\bm{h}_t^{l} + \bm{W_r}\bm{h}_t^{r})),
\end{equation}
where $\bm{h}_t^{l}$ and $\bm{h}_t^{r}$ are agents' higher-level representations from two encoder output. $\bm{W_l},\bm{W_r} \in \mathbb{R}^{d_h \times d_e}, u \in \mathbb{R}^{d_h \times 1}$ are trainable parameters and $d_h, d_e$ are the hidden dimension and encoder output dimension respectively. The logistic sigmoid function $\sigma(\cdot)$ generates the probability for constructing the Bernoulli distribution. Then the binary adjacency matrix $A$ is sampled from this distribution. 
The binary adjacency matrix forms a directed graph, corresponding to the Coord. factor $\mathcal{G}$.
%to obtain the binary adjacency matrix, that is, to construct the Coord. factor $\mathcal{G}$.
The topological order of $\mathcal{G}$ denotes the decision dependency sequence of the agents for interacting with the environments. Here, we denote this graph generation process as $\mathcal{G} \sim \rho_{\varphi}(\bm{h})$.

The acyclicity constraint is a remaining issue. In this work, we also use the penalty terms like~\cite{zheng2018dagsnotears,lachapelle2020gradientdag,zhu2019dagRL} to ensure the acyclicity. The result proposed by~\cite{zheng2018dagsnotears} shows that the directed graph $\mathcal{G}$ with binary adjacency matrix $A$ is acyclic if and only if:
\begin{equation}
\label{eq:dag_constr}
    g(A):=trace(e^{A \circ A})-d=0,
\end{equation}
where $e^{A \circ A}$ is the matrix exponential and $A \circ A$ guarantees the non-negativity. $d$ is the number of nodes in the DAGs. The constraint function $g$ can be any function that satisfies the derivatives of $g$ is computable and $g$ is the measurement of DAGs.
% \jqruan{there is a typo}

Moreover, taking the trade-off between the computing resource and the task performance into account, we propose that the depth of graph structure should be adjustable while dealing with different tasks. 
% The fact in graph theory show that the entry $A^k_{ij}$ of $k$-th power of the adjacency matrix $A$ indicates the number of walks of length $k$ from node $v_i$ to $v_j$. Based on this, 
Therefore, we propose an alternative constraint to control the maximum depth of the generated DAGs as follows.
% We set hyperparameter $k$ as the expected depth of the learned graph structure for a given task. 

\begin{definition}
A square matrix $A$ is Nilpotent Matrix~\cite{Algebra75}, if
\begin{equation*}
    {A^k} = O \ and \ {A^{k - 1}} \ne O, \ \exists k \in {\mathop{\rm \mathbb{Z^+}}} ,
\end{equation*}
\end{definition}
where $O$ is the zero matrix. Also, $A$ is called nilpotent of index $k$.


\begin{proposition}
Let $A$ be the adjacency matrix for a directed acyclic graph. The hierarchy of the DAGs is  denoted as $hire_\mathcal{G}$. $hire_\mathcal{G}$ equals k if $A$ is Nilpotent Matrix of index $k$.
\end{proposition}
\begin{proof} 
Firstly, we prove that the entry $A^k_{ij}$ in $k$-th power of the adjacency matrix $A$ indicates the number of walks of length $k$ from node $v_i$ to $v_j$. Let $\mathcal{L}^l(i,j)$  denote the number of walks of length $l$ from node $v_i$ to $v_j$. When $l=1$, $A^1 = A, a_{ij}=\mathcal{L}^1(i,j)$. Let $b_{ij} =\mathcal{L}^k(i,j)$ denote the $ij^{th}$ entry of $A^k$. We have ${A_{ij}^{k + 1}} = A_{ij}{A_{ij}^k} = {a_{i1}}{b_{1j}} + {a_{i2}}{b_{2j}} + ... + {a_{in}}{b_{nj}} = \sum\nolimits_n {{a_{in}}{b_{nj}}}$, where ${\forall _m} \in [1,n],{a_{im}}{b_{mj}} = {\mathcal{L}^1}(i,m) \cdot {\mathcal{L}^k}(m,j) = {\mathcal{L}^{k + 1}}(i,j)$. So $A_{ij}^{k + 1}$ denote the number of walks of length $k+1$ from $v_i$ to $v_j$. Then:
\begin{equation}
\label{eq:hire_constr}
    \begin{array}{l}
{h^k}(A): = sum({A^k}) = \sum\nolimits_i {\sum\nolimits_j {A_{ij}^k = 0} } \\
{h^{k - 1}}(A): = sum({A^{k - 1}}) = \sum\nolimits_i {\sum\nolimits_j {A_{ij}^{k - 1} > 0} } 
\end{array}.
\end{equation}
The equations represent there is not a walk of length $k$ and there is at least one walk of length $k-1$ from $v_i$ to $v_j$ respectively, that is ${A^k} = O, {A^{k - 1}} \ne O$. We define the hierarchy of the DAGs as the longest path length. Therefore, the hierarchy of the DAGs is $k$ if $A$ is the Nilpotent Matrix of index $k$.
\end{proof}
% Based on the foregoing, we can augment the loss function with $h(A)=h_1(A)-h_2(A)$ to ensure the constraint of the hierarchy while training. 

\textbf{Coord. Critic}. 
To fully take advantage of the extrinsic rewards from the environment to find the useful and distinguishable graph structure, we use the Coord. Critic to evaluate the value of the latent variables which are used to generate the DAGs and directly determine the quality of graph structure.
The Coord. Critic is implemented by a two-layer feed-forward neural network activated by the ReLU units, denoted as $f_{critic}(\bm{h_t})=ReLU(\textit{MLP}\langle \bm{h_t} \rangle)$.

% our critic is a simple 2-layer feed-forward NN with ReLU units, with the
% input being the encoder outputs

% The Critic is trained with a mean squared error between its predictions and the true rewards.

% Based on the foregoing, we can optimize the graph generation policy by the Proposition~\ref{prop:gg}.

\textbf{Training.} Therefore, based on the foregoing, we can optimize the graph generation policy $\rho$ with the $hire_\mathcal{G}=k$ by the following equality-constrained method.
\begin{equation}
\label{eq:cons}
    \begin{array}{l}
\max \ J_R^{\rho } = {\mathbb{E}^{\rho }}\left[ {\sum\limits_{t = 0}^\infty  {{\gamma ^t}{r_t}} } \right] \vspace{2pt} \\
s.t. \ g(A) = 0,{h^k}(A) = 0,{h^{k-1}}(A) > 0
\end{array}
\end{equation}

\begin{proposition}
% The gradient for training the Coord. Actor consists of two terms. The former term denotes the influence on the training of reinforcement learning tasks under the generated graph structure. The latter is the constraint of being a directed acyclic graph.
The gradient for training the graph generation policy $\rho$ is can be derived as follows:
% 
\label{prop:gg}
\begin{equation*}
% \begin{array}{l}
% {\nabla _\varphi }J({\rho ^i}) = {E_{\hat A \sim \rho ( \cdot |s),s \sim p}}\left[ {{\nabla _\varphi }\log \rho (\hat A|s)\sum\limits_{{u^i}} {{{\hat \pi }^i}({u^i}|{o^i},{u^{pa(i) \sim \hat A}}) \cdot } } \right.\\
% \qquad\qquad \left[ {{Q_{{{\hat \pi }^i}}}({o^i},{u^i}) - {{\hat V}_{{{\hat \pi }^i}}}({{\hat o}^i})} \right]\left. { - {\lambda _1}{{({e^{\hat A \circ \hat A}})}^T} \cdot 2\hat A} \right]
% \end{array}
\begin{array}{l}
\begin{array}{*{20}{l}}
{{\nabla _\varphi }J({\rho ^i}) = {E_{s \sim p,A \sim \rho ( \cdot |s)}}\left[ {{\nabla _\varphi }\log \rho (A|s)\sum\limits_{{u^i}} {{{\hat \pi }^i}({u^i}|{o^i},{u^{pa(i) \sim A}}) \cdot } } \right.} \vspace{2px} \\
{\qquad \qquad \left[ {{Q_{{{\hat \pi }^i}}}({o^i},{u^i}) - {{\hat V}_{{{\hat \pi }^i}}}({{\hat o}^i})} \right] - {\lambda _1}{{({e^{A^\circ A}})}^T} \cdot 2A - }
\end{array} \vspace{2px} \\
\qquad \qquad \left. {{\lambda _2}{{\sum\nolimits_{i,j} {\left[ {k{A^k}{A^{ - 1}}} \right]} }_{ij}} + {\lambda _3}{{\sum\nolimits_{i,j} {\left[ {(k - 1){A^{k - 1}}{A^{ - 1}}} \right]} }_{ij}}} \right]
\end{array}
\end{equation*}
\end{proposition}
\begin{proof}
Let ${{{\hat \pi }^i}}$ represent the policy for agent $i$ trained by the Policy Solver. $\varphi$ is the parameter to be solved by the graph generation policy $\rho$ trained by the Coord. Actor.  $g(\cdot)$, $h^k(\cdot)$ and $h^{k-1}(\cdot)$ is the constraint function as shown in Equation~(\ref{eq:dag_constr}) and Equation~(\ref{eq:hire_constr}). 
% ${{{A}_{{{\hat \pi }^i}}}(\cdot)}$ 
${Q_{{{\hat \pi }^i}}}( \cdot )$ denotes the state action function while ${{{\hat V}_{{{\hat \pi }^i}}}(\cdot)}$ is the value function from the Coord. Critic.
% Let $s \in \mathbb{R}^d$ represent the feature vector $(o_t, u_{t-1})$ concisely. 
% We begin by observing that
% Proof of proposition~\ref{prop:one} is provided in appendix A in supplementary. 
We begin by converting the Equation~(\ref{eq:cons}) to the unconstrained problem using the Lagrange relaxation technique~\cite{bertsekas1997nonlinear} as follows.
\begin{equation}
\label{eq:lagrange}
    \max L(\varphi ,{\lambda _1},{\lambda _2},{\lambda _3}) = J_R^{{\rho _\varphi }} - {\lambda _1}g(\mathcal{G}) - {\lambda _2}{h^k}(\mathcal{G}) + {\lambda _3}{h^{k - 1}}(\mathcal{G}),
\end{equation}
where $L$ is the Lagrangian function and $\lambda_i \ge 0, i=1,2,3$ are the Lagrange multipliers. We remark that the Equation~(\ref{eq:lagrange}) converges to Equation~(\ref{eq:cons}) as $\lambda_i$ increases. Correspondingly, the typical effective rule for updating the parameters reads as
\begin{equation}
    {\varphi ^{k + 1}} = {\Gamma _\varphi }\left[ {{\varphi ^k} - {\eta _0}(k){\nabla _\varphi }L({\varphi ^k},\lambda _1^k,\lambda _2^k,\lambda _3^k)} \right], \vspace{-1ex}
\end{equation}
\begin{equation}
\label{eq:lag_mul}
\lambda _i^{k + 1} = {\Gamma _{{\lambda _i}}}\left[ {\lambda _i^k - {\eta _i}(k){\nabla _{{\lambda _i}}}L({\varphi ^k},\lambda _1^k,\lambda _2^k,\lambda _3^k)} \right] \ for \ i = 1,2,3,
\end{equation}
where ${\Gamma }$ is the projection operator defined as~\cite{tessler2018reward_constrain}. The gradients is derived as follows.

\begin{equation*}
\begin{array}{l}
{\nabla _\varphi }L(\varphi ,{\lambda _1},{\lambda _2},{\lambda _3}) = {\nabla _\varphi }\sum\limits_s {{p_{{{\hat \pi }^i}}}(s)\sum\limits_\mathcal{G} {\rho (\mathcal{G}|s)} \sum\limits_{{u^i}} {\left[ {{{\hat \pi }^i}({u^i}|s,\mathcal{G}){A_{{{\hat \pi }^i}}}(s,{u^i})} \right.} } \\
\left. { - {\lambda _1}g(\mathcal{G}) - {\lambda _2}{h^k}(\mathcal{G}) + {\lambda _3}{h^{k - 1}}(\mathcal{G})} \right]\\
 = {\nabla _\varphi }\sum\limits_s {{p_{{{\hat \pi }^i}}}(s)\sum\limits_\mathcal{G} {\rho (\mathcal{G}|s)} \sum\limits_{{u^i}} {\left[ {{{\hat \pi }^i}({u^i}|{o^i},{u^{pa(i)\sim \mathcal{G}}}) \cdot \left[ {{Q_{{{\hat \pi }^i}}}({o^i},{u^i})} \right.} \right.} } \\
\left. {\left. { - {{\hat V}_{{{\hat \pi }^i}}}({{\hat o}^i})} \right] - {\lambda _1}[tr({e^{\mathcal{G}^\circ \mathcal{G}}}) - d] - {\lambda _2}sum({\mathcal{G}^k}) + {\lambda _3}sum({\mathcal{G}^{k - 1}})} \right]\\
 = {\mathbb{E}_{s\sim p,\mathcal{G} \sim \rho ( \cdot |s)}}\left[ {{\nabla _\varphi }\log \rho (\mathcal{G}|s)\sum\limits_{{u^i}} {{{\hat \pi }^i}({u^i}|{o^i},{u^{pa(i)\sim \mathcal{G}}}) \cdot } \left[ {{Q_{{{\hat \pi }^i}}}({o^i},{u^i})} \right.} \right.\\
\left. { - {{\hat V}_{{{\hat \pi }^i}}}({{\hat o}^i})} \right] - {\lambda _1}{({e^{\mathcal{G}^\circ \mathcal{G}}})^T} \cdot 2\mathcal{G} - {\lambda _2}{\sum\nolimits_{i,j} {\left[ {k{\mathcal{G}^k}{\mathcal{G}^{ - 1}}} \right]} _{ij}}\\
\left. { - {\lambda _3}{{\sum\nolimits_{i,j} {\left[ {(k - 1){\mathcal{G}^{k - 1}}{\mathcal{G}^{ - 1}}} \right]} }_{ij}}} \right]
\end{array}
%     \begin{array}{l}
% {\nabla _\varphi }J({\rho ^i}) = {\nabla _\varphi }\sum\limits_{\hat A} {\sum\limits_s {{p_{{{\hat \pi }^i}}}(s)\sum\limits_{{u^i}} {\left[ {{{\hat \pi }^i}({u^i},\hat A|s){A_{{{\hat \pi }^i}}}(s,{u^i}) - {\lambda _1}g(\hat A)} \right]} } } \\
%  = {\nabla _\varphi }\sum\limits_{\hat A} {\sum\limits_s {\sum\limits_{{u^i}} {\left[ {{{\hat \pi }^i}({u^i}|{o^i},{u^{pa(i) \sim \hat A}})\left[ {{Q_{{{\hat \pi }^i}}}({o^i},{u^i}) - {{\hat V}_{{{\hat \pi }^i}}}({{\hat o}^i})} \right] \cdot } \right.} } } \\
% \left. {\rho (\hat A|s) - {\lambda _1}(tr({e^{\hat A \circ \hat A}}) - d)} \right]\\
%  = {E_{\hat A \sim \rho ( \cdot |s),s \sim p}}\left[ {{\nabla _\varphi }\log \rho (\hat A|s)\sum\limits_{{u^i}} {{{\hat \pi }^i}({u^i}|{o^i},{u^{pa(i) \sim \hat A}}) \cdot } } \right.\\
% \left[ {{Q_{{{\hat \pi }^i}}}({o^i},{u^i}) - {{\hat V}_{{{\hat \pi }^i}}}({{\hat o}^i})} \right]\left. { - {\lambda _1}{{({e^{\hat A \circ \hat A}})}^T} \cdot 2\hat A} \right]
% \end{array}
\end{equation*}
\begin{equation*}
    {\nabla _{{\lambda _1}}}L(\varphi ,{\lambda _1},{\lambda _2},{\lambda _3}) =  - {\mathbb{E}_{s\sim p,\mathcal{G}\sim \rho ( \cdot |s)}}\left[ {g(\mathcal{G})} \right]
\end{equation*}
\begin{equation*}
    {\nabla _{{\lambda _2}}}L(\varphi ,{\lambda _1},{\lambda _2},{\lambda _3}) =  - {\mathbb{E}_{s\sim p,\mathcal{G}\sim \rho ( \cdot |s)}}\left[ {{h^k}(\mathcal{G})} \right]
\end{equation*}
\begin{equation*}
    {\nabla _{{\lambda _3}}}L(\varphi ,{\lambda _1},{\lambda _2},{\lambda _3}) =  - {\mathbb{E}_{s\sim p,\mathcal{G}\sim \rho ( \cdot |s)}}\left[ {{h^{k - 1}}(\mathcal{G})} \right]
\end{equation*}
\vspace{-5pt}
\end{proof}
With this, we remark that after considering the influence of various graph structures on the reinforcement learning tasks, we can obtain the optimal graph structure that makes the best response to downstream tasks.





% \begin{figure*}[h]
% \begin{center}
% \includegraphics[width=0.7\linewidth]{fig/exp-overall.png}
% \end{center}
% \caption{Schematics of our framework. The encoder-decoder neural network model is used to generate directed acyclic graph from the observed data with some penalty terms to enforce acyclicity, which are then used to generate the topological order of the action sequence for interacting with the environments and obtain the optimal policy.}
% \label{fig:overview}
% \end{figure*}

\subsection{Policy Solver}

After obtaining the Coord. factor $\mathcal{G}$ from the decision coordinator, we can get the decision sequence according to the parent-child relationship in $\mathcal{G}$, which is a directed acyclic graph. 
Using the prior knowledge of decision sequence, we can further obtain the agent policy for better coordination. 
The architecture of the policy solver module is presented in Fig.\ref{fig:policysolver}. 

\begin{figure}[th!]
\begin{center}
\includegraphics[width=1.05\linewidth]{fig/policysolver1.png}
\end{center}
\caption{The policy solver.}
\label{fig:policysolver}
\end{figure}

Inspired by QMIX~\cite{rashid2018qmix}, we augment the observation $o_t^i$ of each agent $i$ with their last action $u_{t-1}^i$ and their parents' actions $u_t^{pa(i)}$ drawn from the directed acyclic graph $\mathcal{G}$, denoted as ${\hat o}_t^i$.  The objective of agent $i$ is to find the optimal state-action value $Q_t^{i*}({\hat o}_t^i, u_t^i)$. With a slight abuse of notation for brevity to drop $t$, the state-action value function for the agent $i$ is defined as follows.
\begin{equation}
    Q^i({\hat o}^i,u^i) = \mathbb{E}\left[ {\sum\limits_{t = 0}^\infty  {{\gamma ^t}{R_{t + 1}}\left| {{X_0} = {\hat o}^i,{A_0} = u^i} \right.} } \right],{\hat o}^i \in \mathcal{X},u^i \in \mathcal{A},
\end{equation}
where $\mathcal{X}$ and $\mathcal{A}$ represent the augmented state space and the action space respectively.
The optimal state-action value function can be defined by ${Q^{i*}}({\hat o}^i, u^i) = \mathop {\sup }\limits_{\pi^{i}}  {Q^{\pi^i} }({\hat o}^i, u^i)$ as~\cite{szepesvari2010algorithms}.
Correspondingly, the optimal policy $\pi ^{i*}(\cdot|{\hat o}^i)$ is concentrated on the set of actions that maximize $Q^{i*}({\hat o}^i,\cdot)$. 
%To find $Q^*$, 
The fact for the fixed-point equation defined in Eq.\ref{fixedpoint} provides that the optimal $Q^{i*}$, satisfies $T^{i*}Q^{i*}=Q^{i*}$ and $Q^{i*}$ is the unique solution to this fixed-point equation.
\begin{equation}
{T^{i*}}Q^i({\hat o}^i, u^i) = r({\hat o}^i, u^i) + \gamma \sum\limits_{y \in \mathcal{X}} {P({\hat o}^i, u^i,y)\mathop {\sup }\limits_{a' \in \mathcal{A}} Q^i(y,a')},
\label{fixedpoint}
\end{equation}
where $({\hat o}^i, u^i) \in \mathcal{X} \times \mathcal{A}$,  $T^{i*}$ is a nonlinear operator and maximum-norm contraction~\cite{szepesvari2010algorithms}. 

To find $Q^{i*}$, deep Q-network(DQN) is the key method that can be updated by 
${Q^i}({\hat o}^i, u^i) = (1 - \alpha ){Q^i}({\hat o}^i, u^i) + \alpha (r + \gamma {\max _{a'}}{Q^{i^{-}}}({\hat o}^{i{'}},a'))$, 
where $\alpha \in (0,1)$ is the learning rate, 
$\gamma \in (0,1)$ is the discounted factor and $Q^{i^-}$ is the target network. 
For the multi-agent case with distributed observations and actions across $N$ agents, the assumption called Individual-Global-Max (IGM) defined by~\cite{son2019qtran} asserts that $\exists {Q^i}$,
$\mathop {\arg \max }\limits_\textbf{u} {Q_{tot}^*}(\bm{\tau } ,\textbf{u}) = ( {\mathop {\arg \max }\limits_{{u^1}} {Q^1}({\bm{\tau } ^1},{u^1}),}...,\mathop {\arg \max }\limits_{{u^i}} {Q^i}({\bm{\tau } ^i},{u^i}),...,$ \\
${\mathop {\arg \max }\limits_{{u^N}} {Q^N}({\bm{\tau } ^N},{u^N})} )$ holds, where ${\bm{\tau }}$ is the history of the agent. 
Therefore, our policy solver is trained to minimize the following loss which aims to obtain the $Q_{tot}^*$:
\begin{equation}
\label{eq:policy}
    \mathcal{L}(\theta ) = \sum\limits_{j = 1}^b {\left[ {y_j^{tot} - {Q_{tot}}{{((\bm{\tau},\bm{u}^{pa}) ,\bm{u};\theta )}^2}} \right]},
\end{equation}
where the size of the minibatch is $b$ sampled from the replay buffer. ${y^{tot}} = r + \gamma {\max _{\bm{u}'}}((\bm{\tau}',\bm{u}'^{pa}),\bm{u}';{\theta ^ - })$ is the learning target from the target network parameterized by $\theta^-$.



Although we focus on the DQN-based method for the policy solver, the policy-based methods such as MADDPG~\cite{lowe2017maddpg}, MAPPO~\cite{yu2021mappo} are also applicable and the gradient of the policy for the agent $i$ can be written as follows:
\begin{equation}
\begin{array}{l}
{\nabla _{{\theta ^i}}}\mathcal{L}({\theta ^i}) = {E_{{u^i} \sim \pi ( \cdot |{o^i},{u^{pa(i)}}),A \sim \rho ( \cdot |{\tau ^i})}}\left[ {{\nabla _{{\theta ^i}}}\log {\pi _{{\theta ^i}}}({u^i}|{o^i},{u^{pa(i)}})} \cdot \right.\\
\left. \qquad \qquad  {{Q_{{\pi _{{\theta ^i}}}}}({\tau ^i},{u^i})\rho (A|{\tau ^i})} \right].
\end{array}
\end{equation}

\subsection{Algorithm Description}

The main procedures of our approach are illustrated in Algorithm~\ref{algo:nn}, which is the solution of the optimization problem for ${\nabla _{{\theta ^i}}}\mathcal{L}({\theta ^i})$ and ${{\nabla _\varphi }J({\rho})}$. 

% \jqruan{there is an algorithm description.}
\begin{algorithm}
\caption{ACG-MARL}
\label{algo:nn}
% \LinesNumbered 
\textbf{Ensure} agent policy $\pi^i$ and graph generation policy $\rho$;\\
\textbf{Initialize}~$\epsilon,\gamma,M,C$ and replay buffer $\mathcal{D}\leftarrow \emptyset$;\\
\textbf{Initialize}~the parameters $\theta^i$ for the agent policy networks, the target networks $\theta^{i^-}=\theta^i$ for $i=1,...,n$, $\varphi$ for the graph generation network;\\
% step=0, episodes=0;\\
\For {\rm each episode}{
initial state $\leftarrow \{o_0^i\}_{i=1}^n$; // drop $i$ as $\bm{o_0}$ for clarity; \\
\textbf{Initialize} $h_0^{(1)},...,h_0^{(n)}$ for RNN states;\\
\For{\rm each timestep $t$}{
Get $\mathcal{G}_t \sim \rho(\cdot | \bm{o_t})$; \\
Get the topological order $A_t \sim \mathcal{G}_t$ for actions; \\
\For{\rm $i$ in order $A_t$}{
augment the observations as $\hat o_t^i = (o_t^i, u_{t-1}^i, u_t^{pa(i)}) $;\\
sample the action with $\epsilon$-greedy from $Q_t^{\pi^i}(\hat o_t^i, u_t^i;\theta^i)$;\\
Update RNN state $h_{t}^{(1)},...,h_{t}^{(n)}$ $\leftarrow$ $h_{t-1}^{(1)},...,h_{t-1}^{(n)}$ ;\\
Receive reward ${\bf{r}_t}$ and observe next state ${\bf{o}}_{t+1}$; \\
Add transition $\{{\bf{o}}_t, {\bf{u}}_t, {\bf{r}}_t, {\bf{o}}_{t+1}\}$ into $\mathcal{D}$;
}
}

\If{ $episodes > M$}{
sample a minibatch $\mathcal{B}=\{{\bf{o}}_j, {\bf{u}}_j, {\bf{r}}_j, {\bf{o}}_{j+1}\}^M_{j=0}\sim \mathcal{D}$; \\
Update agent policy $\pi^i$ using $\mathcal{B}$ and (\ref{eq:policy});\\
Update graph generation policy $\rho$ using $\mathcal{B}$ and $\frac{1}{n}\sum\nolimits_i {{\nabla _\varphi }J({\rho ^i})}$;\\
Every $C$ steps reset $\theta_i^-=\theta_i$ for $i=1,...,n$;\\
Update Lagrange multipliers using~(\ref{eq:lag_mul});
}
}
\end{algorithm}


Our ultimate goal is to obtain the optimal agent policy $\{\pi^i\}_{i=1}^n$.
% and the intermediate goal is to get the optimal graph generation policy $\rho$. 
The graph generation policy $\rho$ is an intermediate goal, which is used to obtain an excellent graph structure to guide the decision-making sequence among agents to achieve a high degree of multi-agent coordination. 
We use the replay buffer $\mathcal{D}$ for the off-policy updates in a similar manner to DQN~\cite{mnih2015dqn} by applying batch sampling. The Decision Coordinator for generating the graph structure is a pluggable module that can be replaced by other algorithms for solving the DAGs. It should be noted that DAGs are necessary because we need an execution structure that can determine the clear sequence of the actions and therefore it should be directed and not be circular. The Policy Solver is a universal module.
In general, one can choose from a diverse set of cooperative MARL algorithms~\cite{sunehag2018vdn,rashid2018qmix,lowe2017maddpg,yu2021mappo} as the Policy Solver.


% --------------------------------------------------------------------------------------


% \textbf{Training}





